Dual-level Mixup for Graph Few-shot Learning with Fewer Tasks

Graph neural networks have been demonstrated as a powerful paradigm for effectively learning graph-structured data on the web and mining content from it.Current leading graph models require a large number of labeled samples for training, which unavoidably leads to overfitting in few-shot scenarios. Recent research has sought to alleviate this issue by simultaneously leveraging graph learning and meta-learning paradigms. However, these graph meta-learning models assume the availability of numerous meta-training tasks to learn transferable meta-knowledge. Such assumption may not be feasible in the real world due to the difficulty of constructing tasks and the substantial costs involved. Therefore, we propose a SiMple yet effectIve approach for graph few-shot Learning with fEwer tasks, named SMILE. We introduce a dual-level mixup strategy, encompassing both within-task and across-task mixup, to simultaneously enrich the available nodes and tasks in meta-learning. Moreover, we explicitly leverage the prior information provided by the node degrees in the graph to encode expressive node representations. Theoretically, we demonstrate that SMILE can enhance the model generalization ability. Empirically, SMILE consistently outperforms other competitive models by a large margin across all evaluated datasets with in-domain and cross-domain settings. Our anonymous code can be found here.

==> preliminary.tex <==
\section{Preliminary}
Given a graph $\mathcal{G}\!=\!\{\mathcal{V},\mathcal{E},\mathrm{Z},\mathrm{A}\}$, $\mathcal{V}$ and $\mathcal{E}$ represent the sets of nodes and edges, respectively. $\mathrm{Z}\!\in\!\mathbb R^{n\times d}$ is the feature matrix of nodes and $\mathrm{A}\!\in\!\mathbb R^{n\times n}$ is the corresponding adjacency matrix. Our model adheres to the prevalent meta-learning training paradigm, which involves training on sampled tasks. %a per-task basis. %Our model is trained using a task-based approach, which is also the most widely adopted method for training meta-models. %The meta-training tasks $\mathcal{D}_{org}\!=\!\{\mathcal{T}_{t}\}_{t=1}^{\mathrm{T}_{org}}$ are sampled from a task distribution $p(\mathcal{T})$, where each task contains a support set $\mathcal{S}_t\!=\!\{(\mathrm{Z}_{t,i}^s,\mathrm{Y}_{t,i}^s)\}_{i=1}^{n_s}$ and a query set $\mathcal{Q}_t\!=\!\{(\mathrm{Z}_{t,i}^q,\mathrm{Y}_{t,i}^q)\}_{i=1}^{n_q}$, denoted as $\mathcal{T}_t\!=\!\{\mathcal{S}_t,\mathcal{Q}_t\}$. Here, $\mathrm{Z}_{t,i}^\ast$ and $\mathrm{Y}_{t,i}^\ast\!\in\!\mathcal{Y}_{tra}$ denote a labeled node and its corresponding label, where $\mathcal{Y}_{tra}$ denotes the set of base classes. For the meta-testing task $\mathcal{T}_{tes}\!=\!\{\mathcal{S}_{tes},\mathcal{Q}_{tes}\}\!=\!\{\{(\mathrm{Z}_{tes,i}^s,\mathrm{Y}_{tes,i}^s)\}_{i=1}^{n_s}, \{(\mathrm{Z}_{tes,i}^q,\mathrm{Y}_{tes,i}^q)\}_{i=1}^{n_q}\}$, it is composed in the same way as the meta-training task $\mathcal{T}_t$, with the only difference being that the node label belong to the novel class set $\mathcal{Y}_{tes}$, which is disjoint from $\mathcal{Y}_{tra}$, \textit{i.e.}, $\mathcal{Y}_{tra}\!\cap\!\mathcal{Y}_{tes}\!=\!\emptyset$. When the support set $\mathcal{S}_{tes}$ consists of $N$ sampled classes, each with $K$ nodes, we refer to it as an $N$-way $K$-shot problem. Typically, the model is first trained on the meta-training tasks $\mathcal{D}_{org}$. During the meta-testing stage, the model is fine-tuned on $\mathcal{S}_{tes}$ and then is evaluated the performance on $\mathcal{Q}_{tes}$. 
In this work, we mainly focus on few-shot node classification, which is the most prevailing and representative task in graph few-shot learning. Moreover, we highlight that in our focused scenarios, the number of available meta-training tasks sampled from an unknown task distribution is extremely small compared to traditional experimental settings, referred to as \textit{few-shot node classification with fewer tasks}. Our goal is to enable the model to effectively extract meta-knowledge even from such limited tasks, which can generalize to novel tasks in the meta-testing phase. %For better understanding, we summarize the main symbols of this work in \textbf{Appendix} \ref{symbol}.


% $\mathcal{D}_{org}=\{\mathcal{T}_{t}\}_{t=1}^{\mathrm{T}_{org}}, \mathcal{T}_t=\{\mathcal{S}_t,\mathcal{Q}_t\}$, 

% $\mathcal{S}_t=\{(\mathrm{X}_{t,i}^s,\mathrm{Y}_{t,i}^s)\}_{i=1}^{n_s}$, 
% $\mathcal{Q}_t=\{(\mathrm{X}_{t,i}^q,\mathrm{Y}_{t,i}^q)\}_{i=1}^{n_q}$, 

% $\mathcal{S}_t^\prime=\{(\mathrm{X}_{t,i}^{\prime s},\mathrm{Y}_{t,i}^{\prime s})\}_{i=1}^{n_{s^\prime}}$, 
% $\mathcal{Q}_t^\prime=\{(\mathrm{X}_{t,i}^{\prime q},\mathrm{Y}_{t,i}^{\prime q})\}_{i=1}^{n_{q^\prime}}$,

% $\mathcal{T}_t=\{\mathcal{S}_t\cup\mathcal{S}_t^\prime,\mathcal{Q}_t\cup\mathcal{Q}_t^\prime\}$

% $\mathcal{D}_{all}=\mathcal{D}_{org}\cup\mathcal{D}_{aug}$, $\mathcal{D}_{aug}=\{\mathcal{T}_t^{aug}\}_{t=1}^{\mathrm{T}_{aug}}, \mathrm{T}=\mathrm{T}_{org}+\mathrm{T}_{aug}$

%\paragraph{Problem Statement.}
